Control Barrier Functions for Nonholonomic Systems under Risk Signal Temporal Logic Specifications

Temporal logics provide a formalism for expressing complex system specifications. A large body of literature has addressed the verification and the control synthesis problem for deterministic systems under such specifications. For stochastic systems or systems operating in unknown environments, however, only the probability of satisfying a specification has been considered so far, neglecting the risk of not satisfying the specification. Towards addressing this shortcoming, we consider, for the first time, risk metrics, such as (but not limited to) the Conditional Value-at-Risk, and propose risk signal temporal logic. Specifically, we compose risk metrics with stochastic predicates to consider the risk of violating certain spatial specifications. As a particular instance of such stochasticity, we consider control systems in unknown environments and present a determinization of the risk signal temporal logic specification to transform the stochastic control problem into a deterministic one. For unicycle-like dynamics, we then extend our previous work on deterministic time-varying control barrier functions.

==> chapter/problem_formulation.tex <==
\subsection{Problem Formulation}

Consider a dynamical system as given by 
\begin{align}\label{system_noise}
\dot{\boldsymbol{x}}(t)&=f(\boldsymbol{x}(t))+g(\boldsymbol{x}(t))\boldsymbol{u}(t), \; \boldsymbol{x}(0):=\boldsymbol{x}_0
\end{align} 
where $\boldsymbol{x}_0\in\mathbb{R}^n$ is the initial condition and where $\boldsymbol{u}(t)\in\mathbb{R}^m$, $f:\mathbb{R}^n\to\mathbb{R}^n$, and $g:\mathbb{R}^n\to\mathbb{R}^{n\times m}$. 
\begin{problem}
Assume that \eqref{system_noise} is subject to an SITL task $\phi$. Derive a control law  $\boldsymbol{u}(\boldsymbol{x},t)$ so that $(\boldsymbol{x},0)\models \phi$ where $\boldsymbol{x}:\mathbb{R}_{\ge 0}\to \mathbb{R}^n$ is the solution to \eqref{system_noise} under $\boldsymbol{u}(\boldsymbol{x},t)$.
\end{problem}
